Fine-Grained Named Entities for Corona News

Information resources such as newspapers have produced unstructured text data in various languages related to the corona outbreak since December 2019. Analyzing these unstructured texts is time-consuming without representing them in a structured format; therefore, representing them in a structured format is crucial. An information extraction pipeline with essential tasks -- named entity tagging and relation extraction -- to accomplish this goal might be applied to these texts. This study proposes a data annotation pipeline to generate training data from corona news articles, including generic and domain-specific entities. Named entity recognition models are trained on this annotated corpus and then evaluated on test sentences manually annotated by domain experts evaluating the performance of a trained model. The code base and demonstration are available at https://github.com/sefeoglu/coronanews-ner.git.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/problem_setting.tex <==
% \section{Problem Setting}
% Numerous articles in the corona domain have been published on official web pages and newspapers since December 2019. News articles include generic and domain-specific entities, whereas scientific papers contain mostly domain-specific entities. This is because the scientific papers' actual domain comes from science like biomedicine. Therefore, earlier introduced corpora, such as CORD-19~\cite{CORD_19} and LitCovid~\cite{LitCovid_19}, are not adequate to detect recently taken measures and mutations of coronavirus, such as omicron variant, in the news articles. 

% As a result, a new training corpus from up-to-date articles must be constructed to use it in downstream applications. Otherwise, these applications using the outdated corpus might not detect some crucial information in these news articles. Due to these reasons, an annotated corona news corpus is needed for developing qualified applications.
